GeoHopNet: Hopfield-Augmented Sparse Spatial Attention for Dynamic UAV Site Location Problem

The rapid development of urban low-altitude unmanned aerial vehicle (UAV) economy poses new challenges for dynamic site selection of UAV landing points and supply stations. Traditional deep reinforcement learning methods face computational complexity bottlenecks, particularly with standard attention mechanisms, when handling large-scale urban-level location problems. This paper proposes GeoHopNet, a Hopfield-augmented sparse spatial attention network specifically designed for dynamic UAV site location problems. Our approach introduces four core innovations: (1) distance-biased multi-head attention mechanism that explicitly encodes spatial geometric information; (2) K-nearest neighbor sparse attention that reduces computational complexity from $O(N^2)$ to $O(NK)$; (3) a modern Hopfield external memory module; and (4) a memory regularization strategy. Experimental results demonstrate that GeoHopNet extends the boundary of solvable problem sizes. For large-scale instances with 1,000 nodes, where standard attention models become prohibitively slow (over 3 seconds per instance) and traditional solvers fail, GeoHopNet finds high-quality solutions (0.22\% optimality gap) in under 0.1 seconds. Compared to the state-of-the-art ADNet baseline on 100-node instances, our method improves solution quality by 22.2\% and is 1.8$\times$ faster.

==> Makefile <==
# Makefile for GeoHopNet LaTeX paper compilation

# Variables
MAIN = main
TEXFILE = $(MAIN).tex
PDFFILE = $(MAIN).pdf
BIBFILE = references.bib

# LaTeX compiler
LATEX = pdflatex
BIBTEX = bibtex

# Default target
all: $(PDFFILE)

# Compile the main PDF
$(PDFFILE): $(TEXFILE) $(BIBFILE)
	$(LATEX) $(TEXFILE)
	$(BIBTEX) $(MAIN)
	$(LATEX) $(TEXFILE)
	$(LATEX) $(TEXFILE)

# Clean auxiliary files
clean:
	rm -f *.aux *.bbl *.blg *.log *.out *.toc *.lof *.lot *.fls *.fdb_latexmk *.synctex.gz

# Clean all generated files including PDF
cleanall: clean
	rm -f $(PDFFILE)

# Quick compilation (without bibliography)
quick:
	$(LATEX) $(TEXFILE)

# View the PDF (requires a PDF viewer)
view: $(PDFFILE)
	@if command -v evince >/dev/null 2>&1; then \
		evince $(PDFFILE) &; \
	elif command -v okular >/dev/null 2>&1; then \
		okular $(PDFFILE) &; \
	elif command -v xpdf >/dev/null 2>&1; then \
		xpdf $(PDFFILE) &; \
	else \
		echo "No PDF viewer found. Please install evince, okular, or xpdf."; \
	fi

# Help target
help:
	@echo "Available targets:"
	@echo "  all      - Compile the complete paper with bibliography"
	@echo "  quick    - Quick compilation without bibliography"
	@echo "  clean    - Remove auxiliary files"
	@echo "  cleanall - Remove all generated files including PDF"
	@echo "  view     - Open the PDF in a viewer"
	@echo "  help     - Show this help message"

# Phony targets
.PHONY: all clean cleanall quick view help 
